Controllable interaction between photons and distant spins via vacuum Rabi oscillations

Vacuum Rabi oscillations between a single photon and a single spin demonstrate the capability of harnessing light-matter interaction at the level of a single quantum of energy. Since the observation of strong spin-photon coupling in gate-defined quantum dots, probing this interaction in the time-domain has been a major objective. Here, we carefully engineer a device composed of two spatially separated double quantum dots hosting single electron spin qubits and a superconducting cavity to accommodate microwave photons. We observe multiple vacuum Rabi oscillations between each spin qubit and the cavity. By concatenating vacuum Rabi oscillations involving the two spins, an energy excitation in one qubit can be emitted as a photon and then transferred to the other qubit. When a single photon is emitted, the cavity is prepared in a Fock state, leading to an accelerated vacuum Rabi frequency. These results serve as building blocks not only in exploring light-matter interactions, but also in interfacing semiconductor spin qubits to photonic links.

==> numbers.tex <==
Notes: 
1. Everywhere we neglect pure spin dephasing ($\gamma_\phi=0$), such that $T_2^*=2T_1$. 
2. Some numbers can also be found in the Supplementary Table. I included some additional digits here.
3. Talked to Jurgen:
For the averaging, I use the fact that the inner loop always consists of 1e5 repetitions.
Then:
a. For all 2D scans each datapoint is averaged 1e5 times.
b. For all 1D scans each datapoint is averaged 1e5*Ydimension times.

Numbers:
- Magnetic field for spin resonance (Fig 3):
	- Magnitude = 53.4 mT
	- Angle = 9.42 degrees
- Figure 2a (VRO Q1):
	- Fitted vacuum Rabi frequency ($2g_s$) = 27.320628 MHz
	- Fitted relaxation rate $\gamma_1$ = 2.67778 MHz
	- $T_1 = 1/(2\pi\gamma_1[\rm{MHz}])$ = 59.4353397 ns
	- Number of averages: 10e5
- Figure 2b (VRO Q2):
	- Fitted vacuum Rabi frequency ($2g_s$) = 20.123946 MHz
	- Fitted relaxation rate $\gamma_1$ = 2.797216 MHz
	- $T_1 = 1/(2\pi\gamma_1[\rm{MHz}])$ = 56.89761821 ns
	- Number of averages: 10e5
- Figure 2cd (VRO vs detuning 2D):
    - Number of averages: 1e5
- Figure 3c Inset (VRO Q2):
	- Fitted vacuum Rabi frequency ($2g_s$) = 18.793473 MHz
	- Fitted relaxation rate $\gamma_1$ = 2.4559125 MHz
	- $T_1 = 1/(2\pi\gamma_1[\rm{MHz}])$ = 64.80480877 ns
	- Simulated photon number at $t_{int2}$=25 ns -> $p$ = 0.6455338
		- This is then used as initial photon number for the simulation for the swapped VRO Q1
    - Number of averages: 5e5
- Figure 3c (swapped VRO Q1):
	- Fitted vacuum Rabi frequency ($2g_s$) = 17.79491633 MHz
	- Fitted relaxation rate $\gamma_1$ = 2.5999597 MHz
	- $T_1 = 1/(2\pi\gamma_1[\rm{MHz}])$ = 61.21438785 ns
    - Number of averages: 5e5
- Figure 3d (2D state transfer):
	- Number of averages: 1e5
- Figure 4a (accelerated VRO Q1):
	- Manually fitted photon number = 0.65
	- Simulated prepared photon number (vac VRO Q2) = 0.696529
	- Fitted relaxation rate $\gamma_1$ = 2.3734 MHz
	- $T_1 = 1/(2\pi\gamma_1[\rm{MHz}])$ = 67.057849 ns
	- Number of averages: 10e5
- Figure 4b (accelerated VRO Q2):
	- Manually fitted photon number = 0.55
	- Simulated prepared photon number (vac VRO Q1)= 0.672456
	- Fitted relaxation rate $\gamma_1$ = 1.36585 MHz
	- $T_1 = 1/(2\pi\gamma_1[\rm{MHz}])$ = 116.524174 ns
	- Number of averages: 10e5
